Ba-ZebraConf: A Three-Dimension Bayesian Framework for Efficient System Troubleshooting

The proliferation of heterogeneous configurations in distributed systems presents significant challenges in ensuring stability and efficiency. Misconfigurations, driven by complex parameter interdependencies, can lead to critical failures. Group Testing (GT) has been leveraged to expedite troubleshooting by reducing the number of tests, as demonstrated by methods like ZebraConf. However, ZebraConf's binary-splitting strategy suffers from sequential testing, limited handling of parameter interdependencies, and susceptibility to errors such as noise and dilution. We propose Ba-ZebraConf, a novel three-dimensional Bayesian framework that addresses these limitations. It integrates (1) Bayesian Group Testing (BGT), which employs probabilistic lattice models and the Bayesian Halving Algorithm (BHA) to dynamically refine testing strategies, prioritizing high-informative parameters and adapting to real-time outcomes. Bayesian optimization tunes hyperparameters, such as pool sizes and test thresholds, to maximize testing efficiency. (2) Bayesian Optimization (BO) to automate hyperparameter tuning for test efficiency, and (3) Bayesian Risk Refinement (BRR) to iteratively capture parameter interdependencies and improve classification accuracy. Ba-ZebraConf adapts to noisy environments, captures parameter interdependencies, and scales effectively for large configuration spaces. Experimental results show that Ba-ZebraConf reduces test counts and execution time by 67% compared to ZebraConf while achieving 0% false positives and false negatives. These results establish Ba-ZebraConf as a robust and scalable solution for troubleshooting heterogeneous distributed systems.

==> texts/algorithm.tex <==
%\subsection{Bayesian Halving Algorithm (BHA)}
%\label{sec:test-selection-algorithms}
BHA always attains the optimal rates of convergence of the posterior probability value for the true state to 1, no matter which is the true state in the lattice, even under strong dilution effects ~\cite{Tatsuoka2021.01.15.21249894}. The rates of convergence are exponential due to the discrete nature of the model, so that accurate classification is fast.
% This section presents the proposed test selection algorithms, namely Bayesian Graph Halving Algorithm (\textit{BHA})
The key objective for BHA is to systematically identify the true state by selecting pooled tests that exhaustively and systematically partition the lattice model, with test selection based on the current posterior probability distribution. 
%The motivation behind partitioning is that by performing Bayesian updating, the posterior probability mass will increase in corresponding partitions and will decrease in their complements. This implies that the posterior probability mass will accumulate to a single state based on observed test outcomes, which will eventually lead to a correct classification of the true state.
%
% which would arise as a group testing issue specifically when pool sizes get larger. 
% In fact, a theorem in \todo[noline, bordercolor=white]{REV-1} \textcolor{blue}{\cite{Tatsuoka2021.01.15.21249894}} establishes that the BHA partitioning approach based on $\pi_n$ can  achieve optimal rate of convergence of the Bayesian posterior probability value of true state to one almost surely, and that this rate is exponential due to the discrete nature of the classification model.
Note that states are associated with pooled tests, where the subjects depicted as having negative disease status for the state can also comprise a pooled test. Formally, BHA selects a pooled experiment associated with the state that satisfies: 
\begin{equation}
\label{eq:bha}
\begin{aligned}
\underset{s}{\arg \min} \quad &|\sum_{j \in \big \uparrow \! s} \pi(j) - \dfrac{1}{2}|\\
%\textrm{where} \quad & m_n(s) =\sum\limits_{j \in \tilde{s}} \pi_n(j)\\
\end{aligned}
\end{equation}

%\begin{}[BHA Optimality]
%\label{theorem:BHA-optimality}
%A partition to the lattice model through $s$ will obtain the optimal rate of convergence of the Bayesian posterior probability true state for any given true state.
%\end{theorem}

%\textbf{Remove for reviewing?)}
%The detailed proof of Theorem \ref{theorem:BHA} is outside the scope of this paper. However, the intuitive idea here is \textbf{XXX Ben and Curt - Please add several sentences here to describe the idea behind the theorem.}.
%and can be found in \cite{Tatsuoka2021.01.15.21249894}.

where $\pi(j)$ to be the posterior probability of state $j$. 
\bigskip

Figure \ref{fig:halving} illustrates an example of partitioning a 3-subject lattice model through $A$. States colored in green is $\big \uparrow \! A$ and states colored in red is the complement of $\big \uparrow \! A$. As described in Equation \ref{eq:bha}, BHA keeps partitioning through each state to find the state whose up-set and complement divide the posterior probability distribution as equally as possible. 
% The algorithmic implementation of BHA is described in Algorithm \ref{alg:BHA}. 


\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output

% \begin{algorithm}
% \DontPrintSemicolon
  
%   \KwInput{A lattice model $p$}
%   \KwOutput{A pooled test $e$ that minimizes Equation \ref{eq:halving}}
  
%   $min \leftarrow \infty$ \;
%   $m \leftarrow 0$ \;
%   $e \leftarrow null$ \;
%   \For{each state $s$ in $p$}{
%     $m \leftarrow m_n(s)$ \;
%     \If{$|m-0.5| < min$}{
%         $min \leftarrow m$ \;
%         $e \leftarrow s$ \;
%     }
%   }
%   \Return{$e$}

% \caption{BHA}
% \label{alg:bha}
% \end{algorithm}

% \subsubsection{k-BHA: $k$-test Look-ahead Bayesian Graph Halving Algorithm}
% An extension to BHA is the adoption of group testing where multiple tests are selected and performed simultaneously. This can reduce the back and forth involved in preparing pooled samples for testing after observing results. We hence propose a $k$-test look-ahead graph halving algorithm (k-BHA), such that $k  (k > 1)$ pooled tests can be selected for simultaneous testing. Other than improving testing throughput and reducing test stages, $k$-BHA has bee shown to maintain accuracy in classification.

% %The idea behind {\it $k$-BHA} is to partition the posterior probability sum on the lattice model into $2^k$ partitions according to sets of the following form:\\


% Overall, for a lattice model, $k$-BHA can be depicted as an optimization problem by selecting $k$ tests $s_1, \ldots, s_k$ as follows:

% \begin{equation}
% \label{eq:k-halving}
% \begin{aligned}
% \underset{s_1 \dots s_k}{\arg \min} \quad & |\sum_{j \in  s_1 \cap  s_2 \ldots  s_k} \pi_n(j) - 1/2^k| &+ \\ & |\sum_{j \in  s_1 \cap  s_2 \ldots  s_k^c} \pi_n(j) - 1/2^k| &+ \\ &\ldots &+ \\  &|\sum_{j \in  s_1^c \cap  s_2^c \ldots  s_k^c} \pi_n(j) - 1/2^k|\\
% \end{aligned}
% \end{equation}

% %The procedure of k-BHA is described as follows:\\

% %We choose $k$ pooled samples $s_1, \ldots, s_k$ that minimize

% %\begin{align} 
% %\label{eq:k-halving}
% %\begin{split}
% %    &|\sum_{j \in  s_1 \cap  s_2 \ldots  s_k} \pi_n(j) - 1/2^k| \quad + \quad |\sum_{j \in  s_1 \cap  s_2 \ldots  s_k^c} \pi_n(j) - 1/2^k|\\ + \quad &\ldots\\ + \quad &|\sum_{j \in  s_1^c \cap  s_2^c \ldots  s_k^c} \pi_n(j) - 1/2^k|
% %\end{split}
% %\end{align}

% A partitioning example using $k$-BHA with $k = 2$ is illustrated in Figure \ref{fig:2-halving}. Assuming the model is partitioned through states $A$ and $BC$, where $\big \uparrow \! A = \{A, AB, AC, ABC\}$, $\big \uparrow \! A^c = \{B, C, BC, \hat{0}\}$, $\big \uparrow \! BC = \{BC, ABC\}$ and $\big \uparrow \! BC^c = \{A, B, C, AB, AC, \hat{0}\}$. As shown in Figure \ref{fig:2-halving}, states are hence partitioned into four groups, each containing states of $\big \uparrow \! \cap \big \uparrow \! BC = {ABC}$, $\big \uparrow \! A \cap \big \uparrow \! BC^c = {A, AB, AC}$, $\big \uparrow \!A^c \cap \big \uparrow \! BC = \{BC\}$ and $\big \uparrow \! A^c \cap \big \uparrow \! BC^c = \{B, C, \hat{0}\}$ respectively. If the four partitions generated by halving through $A$ and $BC$ contain more evenly distributed posterior probability sums than any other two-state combinations, then $A$ and $BC$ are the desired tests selected by $k$-BHA with $k = 2$.

% %Example \ref{ex:2-BHA} and Algorithm \ref{alg:2BHA} depicts the tests selection function and algorithm for \textit{2-BHA}. Algorithm \ref{alg:k-BHA} depicts the generalized tests selection algorithm for k-BHA.

% %\begin{example}[$k = 2$] \label{ex:2-BHA}

% %This scheme involves selecting $e_1, e_2$ that splits the posterior mass on the lattice model into $2^k = 4$ parts as equally as possible, hence minimizing

% %\begin{align} \label{eq:k-halving-ex}
% %\begin{split}
%  %   & |\sum_{j \in s_1 \cap  s_2} \pi_n(j) - 1/4| \quad + \quad |\sum_{j \in s_1 \cap  s_2^c} \pi_n(j) - 1/4| \\ + \quad & |\sum_{j \in s_1^c \cap s_2} \pi_n(j) - 1/4| \quad + \quad |\sum_{j \in s_1^c \cap s_2^c} \pi_n(j) - 1/4|
% %\end{split}
% %\end{align}
% %\end{example}

% %\begin{algorithm}
% %\DontPrintSemicolon
  
%   %\KwInput{A lattice model $p$}
%   %\KwOutput{2 pools $e_1$ and $e_2$ that minimize Equation %\ref{eq:k-halving-ex}}
  
%   %$min \leftarrow \infty$ \;
%   %$e_1 \leftarrow null$ \;
%   %$e_2 \leftarrow null$ \;
%   %\For{each state $s_1$ in $p$}{
%     %\For{each state $s_2$ in $p$}{
%         %$m_1 \leftarrow \sum\limits_{j \in \tilde{s_1} \cap %\tilde{s_2}} \pi_n(j)$ \;
%         %$m_2 \leftarrow \sum\limits_{j \in \tilde{s_1}^c \cap %\tilde{s_2}} \pi_n(j)$ \;
%         %$m_3 \leftarrow \sum\limits_{j \in \tilde{s_1} \cap %\tilde{s_2}^c} \pi_n(j)$ \;
%         %$m_4 \leftarrow \sum\limits_{j \in \tilde{s_1}^c \cap %\tilde{s_2}^c} \pi_n(j)$ \;
%     %}
%     %\If{$|m_1-\dfrac{1}{4}| + |m_2-\dfrac{1}{4}| + |m_3-\dfrac{1}{4}| %+ |m_4-\dfrac{1}{4}|  < min$}{
%         %$min \leftarrow m$ \;
%         %$e_1 \leftarrow s_1$ \;
%         %$e_2 \leftarrow s_2$ \;
%     %}
%   %}
%   %\Return{$e_1, e_2$}

% %\caption{2-BHA}
% %\label{alg:2BHA}
% %\end{algorithm}

% % The algorithmic implementation of k-BHA is depicted in Algorithm \ref{alg:k-BHA}. 
% Note that in the example described using Figure \ref{fig:2-halving}, to find the two desired states, a total of 64 combinations of tests need to be considered. In general, performing $k$-BHA is $O(2^{kn})$.

% % In general, for a lattice model generated by a $n$-subject pool, performing k-BHA using Algorithm \ref{alg:k-BHA} is $O(2^{kn})$.

% % \begin{algorithm}
% % \DontPrintSemicolon
  
% %   \KwInput{A lattice model $p$}
% %   \KwInput{An integer $k$}
% %   \KwOutput{k pooled tests $e_1$ \dots $e_k$ that minimize Equation \ref{eq:k-halving}}
  
% %   $min \leftarrow \infty$ \;
% %   $e_1, e_2 \dots, e_k \leftarrow null$ \;
% %   \For{each state $s_1$ in $p$}{
% %     \For{each state $s_2$ in $p$}{
% %     \Indent
% %          \State \dots \;
% %     \EndIndent
% %         \For{each state $s_k$ in $p$}{
% %             $m_1 \leftarrow \sum\limits_{j \in \tilde{s_1} \cap \dots \cap \tilde{s_k}} \pi_n(j)$ \;
% %             $\dots$ \;
% %             $m_{2^k} \leftarrow \sum\limits_{j \in \tilde{s_1}^c \cap \dots \cap \tilde{s_k}} \pi_n(j)$ \;
% %         }
% %     }
% %     \If{$m_{total} = |m_1-\dfrac{1}{2^k}| + \dots + |m_k-\dfrac{1}{2^k}|  < min$}{
% %         $min \leftarrow m_{total}$ \;
% %         $e_1 \leftarrow s_1$ \;
% %         $\dots$ \;
% %         $e_k \leftarrow s_k$ \;
% %     }
% %   }
% %   \Return{$e_1, e_2, \dots e_k$}
  
% % \caption{k-BHA}
% % \label{alg:k-BHA}
% % \end{algorithm}



==> texts/architecture.tex <==
\section{Overview of SBGT}
\label{sec:overview}
As illustrated in Figure~\ref{fig:architecture-overview}, the architecture of SBGT is arranged as a top-down layout with three layers.
Each layer contains some modules (big box), and each module is labeled by its designs and implementations as feature boxes (small colored boxes). Note that features colored in red are proposed in this paper, and features colored in blue are adopted from the existing study\cite{tatsuoka_bayesian_2022}.

\textbf{Top layer.} The top layer of SBGT consists of two modules: the lattice model (\S\ref{sec:bit-based-lattice-model}) and BHA (\S\ref{sec:optimizing-bha}). The lattice model is essential in providing micro-functionalities for Bayesian group testing tasks. The current implementation of the lattice model uses hashmap as the core abstraction. In SBGT, we propose \textit{bit-based lattice model}. It leverages an innovative binary-encoded abstraction (\S\ref{ss:binary-encoded-abstraction}) to formulate the lattice model into a self-indexed array and allows for efficient construction/manipulation using bitwise operations (\S\ref{ss:bitwise-operations}). The test selection functionality is established by performing BHA over the lattice model. In SBGT, we propose optimizing BHA, named \textit{Op-BHA} (\ref{ss:op-bha}), which significantly reduces BHA's computational complexity.

\textbf{Middle Layer.} The middle layer of SBGT is tree-based statistical analysis (\S\ref{sec:tree-schemes-for-statistical-analysis}). It relies on the intricate interplay between the top-layer modules, i.e., lattice model and BHA, to construct trees. \cite{tatsuoka_bayesian_2022} proposed the multi-tree scheme (\S\ref{ss:multi-tree}) with several complexity reduction techniques based on the statistical reasoning of Bayesian group testing, i.e., lattice shrinking, the symmetry approach, and the accuracy trade-off approach. We gain insights from these existing designs and propose two new schemes named \textit{the single-tree scheme} (\S\ref{ss:single-tree}) and \textit{the fusion-tree scheme} (\S\ref{ss:fusion-tree}), which are proven to be much more performant in large-scale statistical analyses.

\textbf{Bottom layer.} The bottom layer of SBGT includes our specifically designed data parallelisms and load-balancing techniques that are deeply integrated with Spark's runtime environment. These features allow top- and middle-layer modules to be parallelized efficiently in Spark. In addition to the existing data parallelization technique, i.e., inter-tree parallelism (\S\ref{ss:multi-tree}), we propose two new parallelisms: intra-lattice parallelism (\S\ref{ss:parallel-test-selection}) and inter-lattice parallelism (\S\ref{ss:single-tree}), to effectively accommodate other new features in SBGT. We further propose \textit{workload alignment} and \textit{multi-threading on Spark} to improve each parallelism's load balance.

SBGT is recognized as a high-performance and scalable framework that realizes the workflow of Bayesian group testing using Spark while offering coherent end-to-end designs, implementations, and optimizations throughout each feature. 


% \vspace{-2.0ex}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/architecture-overview.pdf}
    \caption{Architecture overview of SBGT. Features colored in red are proposed in this paper, and features colored in blue are adopted from the existing study in the community\cite{tatsuoka_bayesian_2022}.}
    \label{fig:architecture-overview}
\end{figure}
% \vspace{-2.0ex}

==> texts/lattice-model.tex <==
\section{Bit-based Lattice Model}
\label{sec:bit-based-lattice-model}

% \subsection{Background on Lattice Model}
% \label{ss:background-lattice-model}

Figure~\ref{fig:workflow}b presents the Hasse diagram of a lattice model with 3 subjects: $A$, $B$, and $C$. In Bayesian group testing, the classification objective is to identify the "true" profile that characterizes positive and negative disease status among the individuals being considered for pooling. Given $N$ subjects, there are $2^N$ possible profiles of individual-level negative and positive diagnoses. A natural partial ordering arises among the states through inclusion, with states representing the subset of negative subjects. For example, the top element (state $ABC$) reflects that all subjects are negative, and the bottom element (state $\hat 0$) is the state that all subjects are positive. Other states represent a mix of negatives and positives. Lattices are partially ordered sets that further assume for any two elements, and there is a unique greatest lower bound and unique least upper bound. This structure is key to understanding how statistical discrimination between states can occur in Bayesian group testing. More details on the lattice model are provided in ~\cite{tatsuoka_ferguson_2003,ferguson_tatsuoka_2004,tatsuoka-2005,tatsuoka_2014,tatsuoka_bayesian_2022}.

In the Bayesian framework, for a given profile of the $N$ subjects in terms of their disease status, to obtain its prior probability, we compute the product of the respective individual prior probabilities of their statuses in the profile. These values form a prior probability distribution across the possible states in the lattice model. After a test response is observed, e.g., we pool subjects $A$ and $C$, and the returned test response is positive, state-level test response probability values for that observation are used in the Bayes rule to update prior probabilities to posterior ones. Response distributions depend on pool size and how many subjects in the pool are positive, given a state profile (the dilution effect). States with relatively high probabilities for the observed response will increase their posterior probability values. These posterior probability values thus embody the combined empirical and prior evidence as to which state in the classification model is true.

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.3\columnwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{figures/lattice-model.pdf}
%          \caption{Lattice Model}
%          \label{fig:lattice-model}
%      \end{subfigure}
%      %\hfill
%      \hspace{3.0ex}
%      \begin{subfigure}[b]{0.3\columnwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{figures/halving.pdf}
%          \caption{BHA}
%          \label{fig:halving}
%      \end{subfigure}
%      \caption{\small{\ref{fig:lattice-model}} presents the Hasse diagram of a lattice model with 3 Subjects $A, B$ and $C$. \small{\ref{fig:halving}} depicts an example of partitioning the lattice model through state $A$.}
%      \label{fig:halving-and-2-halving}
% \end{figure}

\subsection{Binary-encoded Abstraction}
\label{ss:binary-encoded-abstraction}
The existing implementation uses \texttt{HashMap} and key-value pairs \texttt{<state:String, prob:Double>}, e.g., \texttt{<"AC", 0.05>} as the core abstraction of lattice models. This design is natural as each state in a lattice model is associated with a prior/posterior probability and requires frequent access and modification. However, when a lattice model could comprise over 1 billion states ($N = 30$), this design becomes mediocre due to the innate deficiency of hashmap, such as memory overhead, slowness in computing hash functions, and performance instability due to hash collisions. Considering our mission is to improve the performance of Bayesian group testing by over three magnitudes, and the lattice model plays an essential role that every other component relies on, we conclude that optimizing the existing design is unlikely to achieve our goal.

While exploring the lattice model's design space, we made tryouts in multiple data structures, such as Trie, segment tree, and directed acyclic graph (DAG). However, each has had its known limitation, and none could capture a natural abstraction for the lattice model. Therefore, our tryouts only led to either slight improvement or even worse performance than the hashmap-based design in the current study.

Motivated by the similar partially ordered structure between a lattice model and a power set, we propose a \textit{binary-encoded abstraction} for representing lattice models. This abstraction inherently formulates a bijection between the set of states and a power set, allowing efficient \textit{self-indexing} of each state for accessing its associated prior/posterior probability using binary numbers. The following example describes this process:

\begin{exmp}
\label{ex:bitwise}
Recall the lattice model from Figure \ref{fig:workflow}b. The encoding function uses 1 bit to acknowledge the presence of each subject such that each state is encoded into a binary number with 3 bits, e.g., $AB \rightarrow \{110\}$, $BC \rightarrow \{011\}$. All states hence are subsequently mapped into the power set of $2^{\{111\}} = \{\{000\}, \{001\}, \{010\}, \{011\}, \{100\}, \{101\}, \{110\}, \{111\}\}$, formulating a \textit{bijection} with the lattice model. As visualized in Figure \ref{fig:bit-representation}, by constructing an array of size $2^N$, $N = 3$, we can store and access the corresponding posterior probability of each state by translating its binary encoding to decimal, e.g., $AC$ is encoded as \{101\} and translated to decimal number 5 (incidentally, this translation is only necessary by human, but not for a computer, which makes the binary-encoded abstraction even more appealing), its prior/posterior probability is hence stored and can be accessed at index 5 of the array.
\end{exmp}

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{figures/binary-presentation.pdf}
    \caption{Illustration of the bijection between a lattice model and a power set through binary-encoding abstraction, allowing states to be self-indexed in an array.}
    \label{fig:bit-representation}
\end{figure}
% \vspace{-2.0ex}

\subsection{Bitwise Operations}
\label{ss:bitwise-operations}

The binary-indexed abstraction of lattice models promotes high-performance and concise bitwise operations to manipulate lattice models. For better illustration, we first define a key concept from order theory named \textit{up-set} as follows:

\begin{definition}[Up-set of a state in a lattice]
\label{def:up-set}
For a state $s$ in the lattice, the up-set $\big \uparrow \! s$ is the subset of states within the lattice that is at least as great as (i.e., contain) $s$.
\end{definition}

The computation of up-set is critical in conducting test selections using BHA, which will be discussed in more detail in \S\ref{sec:optimizing-bha}. In the hashmap-based abstraction, determine if state $s_1$ is an up-set of state $s_2$ requires calling \texttt{$s_1$.containsAll($s_2$)}, which takes $O(\text{deg(} s_2 \text{)} \cdot \text{deg(} s_2 \text{)})$. Whereas in the binary-indexed abstraction, since each state is self-indexed, a simple bitwise AND: \texttt{$s_1$ \& $s_2$ == $s_2$}, will suffice the checking, which is theoretically faster than arithmetic addition. 

Another benefit of using bitwise operations on binary-indexed abstraction is that it allows for more logically elegant algorithms for many performance-critical tasks. We illustrate one such task in Example~\ref{ex:find-up-set}. Its usage will be further described in \S\ref{ss:op-bha}.
% One such task is collecting all up-set elements for a given state and calculating their posterior probability summation. We show that an actively generating the up-set using bitwise operations can significantly improve the performance over exhaustive traversal.

\begin{exmp}
\label{ex:find-up-set}
Suppose we want to find $\big \uparrow \! C$, $C$ is 001 (decimal: 1) in binary-indexed abstraction. The absent subjects are $A$ (binary: 100) and $B$ (binary: 010). This can be achieved by actively generating the power sets of both absent subjects in binary, which are $2^{\{\{100\}, \{010\}\}} = \{\{000\}, \{100\}, \{010\}, \{110\}\}$, respectively. Summed by the binary encoding of $C$ ($\{\{001\}$), we get $\{\{001\}, \{101\}, \{011\}, \{111\}\}$, which is equivalent to $\{C, AC, BC, ABC\}$, or $\big \uparrow \! C$. 

\todo[noline, bordercolor=white]{REV-ALL} \textcolor{blue}{Subroutine \texttt{up\_set()} in Algorithm~\ref{alg:test-selection} depicts the algorithmic procedure of this task, where the binary encoding of each element in $\big \uparrow \! s$ is generated in line 35. The complexity of this subroutine is $n \cdot 2^n$ for $s$, where $n = N - \text{cardinality(}s\text{)}$. This subroutine generally has a much lower complexity than the exhaustive traversal approach used in~\cite{tatsuoka_bayesian_2022}, which takes $O(2^N)$.}
\end{exmp}


We summarize the binary-encoded abstraction and bitwise operations as the bit-based lattice model. Note that due to its higher abstraction in biostatistical reasoning and lower perceptibility from complex bitwise operations, the bit-based lattice model is much less intuitive, which burdens programming efforts. We also face significant challenges in seamlessly integrating the bit-based lattice model into other new and existing designs. For example, \cite{tatsuoka_bayesian_2022} proposes the lattice shrinking technique that can sequentially eliminate any classified subjects from the lattice model after updating its posterior probability distribution, drastically reducing model complexity, e.g., each classified subject help reduce the complexity of the lattice model by half. However, using the binary-indexed abstraction becomes troublesome, as it does not ``localize'' a state naturally. To illustrate, $ABC$ is represented as \{111\}. If $B$ is eliminated from the lattice model, then $AC$ becomes binary \{11\}, and it is now impossible to identify if \{11\} represents $AB$ or $BC$ or $AC$ in different contexts. To address this issue, an integer is used as a state locality look-up flag: e.g., when $B$ is classified, we change the flag from 0 to 2, indicating binary \{010\} (or $B$) is classified, which helps identify \{11\} as $AC$. Despite higher design complexity, the bit-based lattice model significantly improves the all-around performance for Bayesian group testing. At $N = 25$, we see up to 376x faster manipulation speed and 96.2\% less memory overhead by using the bit-based lattice model than the existing hashmap-based lattice model. A detailed performance evaluation comparing the two is depicted in \S\ref{ss:lattice-model-benchmark}.


==> texts/op-bha.tex <==
\section{Optimizing Bayesian Halving Algorithm}
\label{sec:optimizing-bha}

% \subsection{Backgroud on BHA}
% \label{ss:backgroud-bha}

BHA is the optimal strategy for guiding test selections using lattice models. To understand BHA, recall Definition~\ref{def:up-set}, a practical interpretation of an up-set in a lattice model under group testing is as follows: $\big \uparrow \! ABC$ is all the states for which a pool of $A$, $B$, and $C$ would contain only negative subjects, $\big \uparrow \! A$ is all the states such that $A$ is negative, etc. Conversely, the complement of the up-set of $\big \uparrow \! ABC^c = \{AB, AC, BC, A, B, C, \hat{0}\}$ represents states for which a pooled test $ABC$ would contain at least one positive sample. Similarly, $\big \uparrow \! A^c = \{BC, B, C, \hat{0}\}$ is comprised of the states for which an individual test of a sample from subject $A$ is likely to be positive, etc. Therefore, the up-set of a state and its complement generate a partition of the classification states based on whether the corresponding pooled test would contain all negatives or some positives. 

The key objective of BHA is to systematically partition the lattice model based on the current posterior probability distribution on the lattice. By partitioning as close to half as possible, the sum of posterior probabilities, known as \textit{posterior probability mass} (or $m(s)$ for a state $s$), will increase in one of the two partitions and decrease in the other. This property systematically implies that the posterior probability mass will quickly accumulate to a single state. The following lemma gives the correctness and optimality of BHA.

\begin{lemma} [Correctness and optimality of BHA]
\label{lemma:bha}
\todo[noline, bordercolor=white]{REV-ALL}
\textcolor{blue}{\textit{BHA attains the optimal rates of convergence of the Bayesian posterior probability for correctly classifying the true state to 1 almost surely, regardless of the true state, and even under strong dilution effects.}}
\end{lemma}

\begin{proof}
\textcolor{blue}{BHA's correctness and optimality are given in~\cite{tatsuoka_bayesian_2022}.}
\end{proof}

\noindent Example~\ref{ex:halving} below depicts the process of conducting BHA on a lattice model.
\begin{exmp}
\label{ex:halving}
Figure~\ref{fig:workflow}c visualizes a partition through state $A$ on a 3-subject lattice model. Green states represent $\big \uparrow \! A$ and red states represent $\big \uparrow \! A^c$. If $m(A)$ (the sum of posterior probabilities of green states) is the closest to 0.5 among any other states, then $A$ is the desired test selection.
\end{exmp} 

\todo[noline, bordercolor=white]{REV-ALL} BHA finds the desired test selection by traversing and partitioning across all states. \textcolor{blue}{Depending on how $m(s)$ is calculated, i.e., exhaustive traversal used in~\cite{tatsuoka_bayesian_2022} or our proposed active generation discussed in Example~\ref{ex:find-up-set}, the overall complexity of BHA can reach $O(2^{2N})$ or $\sum_{n = 0}^{N}{\binom{N}{n} \cdot n \cdot 2^{n}}$. Quantitatively, for $N = 30$, BHA needs to iterate and compute through over 1 billion states ($2^{30}$) for over $1.15 \times 10^{18}$ ($2^{60}$) times using exhaustive traversal, or $3.7 \times 10^{15}$ times using active generation.} The high complexity and large amount of computations for large $N$ motivate us to further explore the design spectrum of BHA beyond mathematical reasoning.

\subsection{Op-BHA Algorithm}
\label{ss:op-bha}

\textcolor{blue}{We give the definition of \textit{down-set} to assist the illustration of our proposed Op-BHA algorithm.}

\begin{definition}[\textcolor{blue}{Down-set of a state in a lattice}]
\label{def:down-set}
\textcolor{blue}{For a state $s$ in the lattice, the down-set $\big \downarrow \! s$ is the subset of states within the lattice that is at most as great as (i.e., are contained by) $s$.}
\end{definition}

\noindent \textcolor{blue}{A critical observation between up-set/down-set and posterior probability mass is summarized as the following theorem.}

\begin{theorem}[\textcolor{blue}{Partial ordering of posterior probability masses in a lattice}]
\label{theorem:1}
\textcolor{blue}{\textit{For states $a$ and $b$ in a lattice model, $m(a) < m(b)$ if $a \in (\big \uparrow \! b \setminus b)$, and $m(a) > m(b)$ if $a \in (\big \downarrow \! b \setminus b)$. $m(a)$ and $m(b)$ are the posterior probability masses of $a$ and $b$.}}
\end{theorem}
\begin{proof}
\textcolor{blue}{Suppose $a \in (\big \uparrow \! b \setminus b)$ and let \{$a_1$, $a_2$, \dots, $a_n$\} = $\big \uparrow \! a$. By Definition~\ref{def:up-set}, $\forall a_i$, $i = 1 \dots n$, $a_i$ is at least as great as $a$. Since $a$ is also at least as great as $b$ and $a \neq b$, $a$ is greater than $b$. It then follows $\big \uparrow \! a \subset \big \uparrow \! b$. Since Bayesian probabilities are always positive, we have $m(a) < m(b)$. The other direction, i.e., $m(a) < m(b)$ does not necessarily mean $a \in (\big \uparrow \! b \setminus b)$, is proved by a counterexample using the 3-subject lattice model shown in Figure~\ref{fig:workflow}b: let subject $A$'s prior probability be 0.1 and $B$'s prior probability be 0.05, then initially, $m(A) = 0.9$ and $m(B) = 0.95$. $m(A) < m(B)$ but $A \notin \big \uparrow \! B$. The proof for down-set follows similarly and is omitted.}
\end{proof}

\todo[noline, bordercolor=white]{REV-ALL}\textcolor{blue}{Theorem~\ref{theorem:1} reveals the opportunity of reducing the number of states necessitated by BHA. Specifically, when traversing each state $s$ in a lattice model, if $m(s) < 0.5$, it is safe to skip calculating posterior masses for all elements in $\big \uparrow \! s$; and if $m(s) > 0.5$, we can otherwise skip calculating posterior masses for all elements in $\big \downarrow \! s$. This concludes the key idea of Op-BHA, and we prove its correctness below.}

\begin{theorem}[\textcolor{blue}{Correctness of Op-BHA}]
\label{theorem:2}
\textcolor{blue}{\textit{Op-BHA is equivalent to BHA and also attains the optimal rates of correctness.}}
\end{theorem}
\begin{proof}
\textcolor{blue}{The proof is obtained by contradiction. Suppose BHA finds the correct test selection $s_c$ for a lattice model of size $N$, it follows that $min\{|m(s_1) - 0.5|, \dots, |m(s_c) - 0.5|, \dots, |m(s_{2^N}) - 0.5|\} = |m(s_c) - 0.5|$. Assuming Op-BHA finds a different test selection $s_e$, such that $s_e \neq s_c$. It implies that $s_c$ is skipped by Op-BHA. If $m(s_c) < 0.5$, then by Op-BHA, $m(s_e) < 0.5$ and $s_c \in \big \uparrow \! s_e$. Combined with Theorem~\ref{theorem:1}, we have $m(s_c) < m(s_d) < 0.5$ and hence $|m(s_e) - 0.5| < |m(s_c) - 0.5|$, which suggests $s_e$ is the correct test selection, contradicting the fact. The proof for $m(s_c) > 0.5$ is similar and is omitted. It then follows by Lemma~\ref{lemma:bha} and proves the theorem.}
\end{proof}

% A useful observation from the posterior probability mass is that, for two states $a$ and $b$, if $a \in \big \uparrow \! b$, then $m(a) < m(b)$ as $\big \uparrow \! a \subset \big \uparrow \! b$. More specifically, if $m(s) < 0.5$ for some state $s$, then we can skip evaluating $\big \uparrow \! s$, as $m(s_i) < m(s) \forall s_i \in \big \uparrow \! s$, meaning their posterior probability masses are farther from 0.5 than $m(s)$. Conversely, if $m(s) > 0.5$, we can skip evaluating ${s_i : s \in \big \uparrow \! s_i}$ ($\{s_i\}$ is also known as the down-set of $s$, denoted as $\big \downarrow \! s$). Based on this fact, we propose an algorithmic optimization for BHA, namely \textit{Op-BHA}.

\noindent An example of potential computation savings of Op-BHA is illustrated as follows.
\begin{exmp}
\label{ex:op-bha-savings}
Let $N = 30$ and every subject has a prior risk level of 0.02. Suppose Op-BHA first partitions through the topmost state $t$ (the state that identifies all subjects are negative). Since $m(t) \approx 0.545 > 0.5$, it will skip evaluating $\big \downarrow \! t \setminus t$, which comprises all remaining states in the lattice model. We thus find the correct test selection by evaluating only one state.
\end{exmp}

\todo[noline, bordercolor=white]{REV-4}\textcolor{blue}{Algorithm~\ref{alg:test-selection} describes the three-phase process for performing a test selection using Op-BHA over a bit-based lattice model. Phase 1 is the one-time prerequisite procedure of constructing a lattice model, and Phase 3 is the recurring postrequisite procedure of updating the lattice model's posterior probability distribution before performing the next Op-BHA. Lines 10 and 13 - 16 comprise BHA's primary computational tasks and are shared by Op-BHA. The rest of Phase 2 represents exclusive algorithmic designs for Op-BHA, and here we focus on them in detail. 1) In line 7, we construct a checklist for tracking each state's traversal status, i.e., skippable or unevaluated. The list is implemented using \texttt{BitSet}, which internally uses an \texttt{Int64} array, where each integer can store statuses for 64 states. We choose over a \texttt{Boolean} array as it only consumes 1/8 the memory. 2) In line 10, we propose a fixed traversal strategy aiming to maximize the number of skippable states. Specifically, the traversal starts from the topmost and bottommost states in the lattice model as they can potentially skip all remaining states, and gradually traverse to the middle states, i.e., states with cardinalities $N/2$ assuming $N$ is even, as each middle state can only reduce up to $2^{N/2}$ states. 3) In line 20, the implementation of \texttt{down\_set()} subroutine follows similarly with \texttt{up\_set()} subroutine with minor changes and is hence omitted. Its algorithmic complexity shares the same formula as \texttt{up\_set()} discussed in Example~\ref{ex:find-up-set} but differs in that $n$ = cardinality($s$). 4) To better illustrate \texttt{Op-BHA()}, each subroutine depicted in Phase 2 uses $O(2^n)$ extra space for storing the up-set/down-set, which is eliminated in the real implementation as each generated state can be consumed immediately. The implementation also adopts  various optimizations to facilitate performance, such as reordering nested loops to alleviate I/O bottlenecks and reusing hot data to improve cache hits.}

\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\SetKwComment{Comment}{$\triangleright$ }{}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\newcommand{\algrule}[1][.8pt]{\par\vskip.25\baselineskip\hrule height #1\par\vskip.25\baselineskip}
\SetKwProg{myproc}{Procedure}{}{}
\SetKwProg{mysubroutine}{Subroutine}{}{}

\begin{algorithm}
\small
\DontPrintSemicolon
  \KwInput{$prior\_prob[N]$}
  \KwOutput{$selection$}
  $prob\_dist[2^N]$ \Comment*[r]{\textnormal{probability distribution}}
  
  \algrule
  \nonl \textit{Phase 1 - Construct Lattice Model} \;
  \algrule
  \myproc{\proc{BUILD\_MODEL(prior\_prob, prob\_dist)}}{
    \For{i=0; i $< 2^N$; ++i}{
        \For{j=0; j $< N$; ++j}{
            i \& 1 $<<$ j == 0 ? $prob\_dist[i] *= prior\_prob[j]$ : $prob\_dist[i] *= 1 - prior\_prob[j]$
        }
    }
  }

  \algrule
  \nonl \textit{Phase 2 - Op-BHA} \;
  \algrule
  \myproc{\proc{Op-BHA(prob\_dist)}}{
    $chklist[2^N]$ \Comment*[r]{\textnormal{track skippable states}}
    $min \leftarrow \infty$ \Comment*[r]{\textnormal{track prob mass closest to 0.5}}
    \textcolor{blue}{$n \leftarrow N - cardinality(s)$ \;}
    \For{\textcolor{blue}{\textit{state s from topmost \& bottommost to middle}}}{
        \If{$chklist.get(s)$}{continue \Comment*[r]{\textnormal{state evaluated / skipped}}} 
        \textcolor{blue}{$mass = calc\_mass(s, prob\_dist)$ \Comment*[r]{\textnormal{$O(n$$\cdot$$2^n)$}}}
        \If{$|mass-0.5| < min$ } {
            $min \leftarrow mass$ \;
            $selection \leftarrow i$ \;
        }
        \uIf{$mass < 0.5$}{
            \textcolor{blue}{$chklist.set(up\_set(s))$ \Comment*[r]{\textnormal{$O(n$$\cdot$$2^n)$}}}
        }
        \ElseIf{$mass > 0.5$}{
            \textcolor{blue}{$chklist.set(down\_set(i))$ \Comment*[r]{\textnormal{$O$(($N$-$n$)$\cdot$$2^{N-n})$}}}
        }
    }
    \Return{$selection$}
  }
  
  \mysubroutine{\proc{\textcolor{blue}{calc\_state\_mass(s, prob\_dist)}}}{
    \textcolor{blue}{$mass \leftarrow 0$, $n \leftarrow N - cardinality(s)$ \;}
    \For{\textcolor{blue}{i = 0; i $< 2^n$; ++i}}{
     \textcolor{blue}{$mass$ += $prob\_dist[up\_set[i]]$ \;}
    } 
    \Return{\textcolor{blue}{$mass$}}
  }

  \mysubroutine{\proc{\textcolor{blue}{up\_set(s)}}}{
    \textcolor{blue}{$n \leftarrow N - cardinality(s)$, $up\_set[2^n]$\;}
    \textcolor{blue}{$absent\_subj[n]$ \Comment*[r]{\textnormal{correct values filled}}}
    \For{\textcolor{blue}{i = 0; i $< 2^n$; ++i}}{
     \textcolor{blue}{$ind \leftarrow s$ \;}
     \For{\textcolor{blue}{j = 0; j $< n$; ++j}}{
        \If{\textcolor{blue}{$i$ \& $(1 << j)$}}{
            \textcolor{blue}{$ind$ += $absent\_subj[j]$ \;}
        }
     }
     \textcolor{blue}{$up\_set[i]$ = $prob\_dist[ind]$ \Comment*[r]{\textnormal{$ind \in \big \uparrow \! s$}}}
    } 
    \Return{\textcolor{blue}{$up\_set$}}
  }
  

  \algrule
  \nonl \textit{Phase 3 - Update \& Shrink Lattice Model} \;
  \algrule
  \myproc{\proc{UPDATE\_SHRINK\_MODEL(selection, response, prob\_dist)}}{
    \For{i=0; i $< 2^N$; ++i}{
        \uIf{\textcolor{blue}{response == negative}}{
            \textcolor{blue}{$prob\_dist[i]$ *= $dilution(i, selection, response)$ \;}
        }
        \ElseIf{\textcolor{blue}{response == positive}}{
            \textcolor{blue}{$prob\_dist[i]$ *= $1 - dilution(i, selection, response)$ \;}
        }
    }
    $normalize(prob\_dist[i])$ \Comment*[r]{\textnormal{normalize distribution}}
    $shrink(prob\_dist[i])$ \Comment*[r]{\textnormal{if subject(s) is classified}}
  }

\caption{Test Selection Using Op-BHA}
\label{alg:test-selection}
\end{algorithm}

\todo[noline, bordercolor=white]{REV-ALL}\noindent \textcolor{blue}{\textbf{Complexity analysis}, \texttt{Op-BHA()} in Algorithm~\ref{alg:test-selection} clearly illustrates the dynamic computational complexity at each loop, i.e., $O(0)$, $O(n$$\cdot$$2^n)$ or $O(n$$\cdot$$2^n$+$(N-n)$$\cdot$$2^{N-n})$. Besides $N$, the aggregated complexity also depends on the posterior probability distribution, which is determined by multiple factors, such as the prior probability information, the ground truth (true state of subjects), test responses, and dilution effects. The enormous degrees of freedom in estimating the posterior probability distribution have prohibited a general-case complexity of Op-BHA from being deduced. However, it is clear that Op-BHA's complexity is at most as complex as BHA, i.e., $\sum_{n = 0}^{N}{\binom{N}{n} \cdot n \cdot 2^{n}} \approx O(2^{2N})$, which presents extremely rare cases such that almost every states has to be evaluated. On the other hand, from Example~\ref{ex:op-bha-savings}, which in fact demonstrates the maximum possible state reduction, we can see Op-BHA's complexity is bounded below by $\Omega(2^N)$.}

\subsection{Parallelzing Op-BHA}
\label{ss:parallel-test-selection}
Besides reducing algorithmic complexity, parallelizing Op-BHA provides another promising passage toward speeding up test selections. We propose parallelizing Op-BHA \todo[noline, bordercolor=white]{REV-4}\textcolor{blue}{using a multi-staged MapReduce programming model based on Spark}, namely \textit{intra-lattice parallelism}. \textcolor{blue}{Note that the design of intra-lattice parallelism is not limited to a data parallelism model as we use. It can be easily ported to other parallel programming models such as message passing (MPI) or partitioned global address space (PGAS).} Figure \ref{fig:intra-lattice-parallelism} describes the multi-staged MapReduce model: the master first broadcasts the posterior probability distribution of the lattice model to workers. Next, it generates a list of yet-to-be-evaluated states, known as \textit{candidate states}, based on the existing checklist. The master then dispatches a chunk of candidate states to workers using \texttt{map()} so that each worker can perform line 11-20 of Algorithm~\ref{alg:test-selection} on given candidate states. Note that when each worker finishes computation, not only does it return to the master a temporarily desired \textit{test selection}, but also an updated checklist indicating which states can be further omitted. These returned results are then processed using \texttt{reduce()}, i.e., the returned test selections are reduced by examining line 14-16 of Algorithm~\ref{alg:test-selection}, and the checklist is reduced by bitwise OR. This concludes the MapReduce stage. If the master detects more candidate states, i.e., the checklist's cardinality does not equal $2^N$, it starts another stage of the procedure until no candidate states are available.

\todo[noline, bordercolor=white]{REV-1}\textcolor{blue}{Differed from the serial algorithm described in Procedure \texttt{Op-BHA()} of Algorithm~\ref{alg:test-selection}, where the checklist is updated on the fly in a shared memory view, the checklist in intra-lattice parallelism is only updated after evaluating multiple states' posterior probability masses after each stage, meaning duplicated computation is inevitable.} Therefore, the chunk size $C$ will play an essential role in the overall performance of intra-lattice parallelism, where a smaller $C$ can result in faster evaluation and more effective state reduction per stage. However, it will potentially increase the number of total stages, hence suffering from more scheduling and data overheads. On the other hand, a larger $C$ may reduce savings from fewer skipped states and a more severe load imbalance because executors can skip different amounts of candidate states. Therefore, there is no one-size-fits-all choice for $C$ as there is no fixed optimal design for varied posterior probability distributions. \todo[noline, bordercolor=white]{REV-1}\textcolor{blue}{Our implementation uses $C = 2^{N/2 + 8}$ based on heuristics to reach a ``sweet point'' between balancing loads and alleviating various overheads while achieving significant workload reduction for Op-BHA}.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/intra-lattice-parallelism.pdf}
    \caption{Intra-lattice parallelism using multi-staged Map-Reduce. The master dispatches tasks at each execution stage as a chunk of candidate states to executors after collecting and processing the checklist returned from the last stage.}
    \label{fig:intra-lattice-parallelism}
\end{figure}

\noindent \textbf{Multithreading on Spark}, we propose shared memory inside each worker to improve the load balance of intra-lattice parallelism. We use a customized fork-join pool to leverage the famous work-stealing algorithm~\cite{10.1145/324133.324234}. This algorithm allows a thread to ``steal'' unfinished tasks from other threads, which is ideal for executing algorithms with dynamic workloads like Op-BHA. Additionally, multithreading on Spark also reduces the number of concurrent tasks while maintaining high degrees of parallelism. It also effectively decreases data communication overheads to improve the scaling efficiency for performing test selections that guide optimal pooling strategies.

\todo[noline, bordercolor=white]{REV-ALL}\noindent \textcolor{blue}{\textbf{Complexity analysis}, suppose $p$ processes are used for intra-lattice parallelism, the complexity of intra-lattice parallelism is bounded above by $O(2^{2N} / p)$, as it assumes almost no states are reduced. the lower bound of intra-lattice parallelism remains at $\Omega(2^N)$, because as illustrated in Example~\ref{ex:op-bha-savings}, there is only one process which holds the topmost state is performing effective state reduction, while the rest $p-1$ processes are in fact performing duplicated computation.}

% \todo[noline, bordercolor=white]{REV-ALL}\noindent \textcolor{blue}{\textbf{Correctness and complexity analysis}, intra-lattice parallelism is analogous to Op-BHA except the checklist is updated only after every MapReduce stage. After the reduce operation, the $C$ newly evaluated states will produce an identical checklist as the one produced by Op-BHA. So intra-lattice parallelism always retains equivalent results as Op-BHA and hence is correct. To illustrate intra-lattice parallelism's complexity, suppose $p$ processes are used for intra-lattice parallelism, the complexity of intra-lattice parallelism is bounded above by $O(2^{2N} / p)$, as it assumes almost no states are reduced. the lower bound of intra-lattice parallelism remains at $\Omega(2^N)$, because as illustrated in Example~\ref{ex:op-bha-savings}, there is only one process which holds the topmost state is performing effective state reduction, while the rest $p-1$ processes are in fact performing duplicated computation.}
% Quantitatively, suppose for a given probability distribution, the workload complexity for evaluating a state $i$ using the proposed traversal strategy is $w_i$, and Op-BHA evaluates $k$ states before finishing. We conclude that the overall computational complexity will be bounded below by $(\sum_{s = 1}^{\lceil k / C \rceil} \sum_{i=1}^{p}\sum_{j=1}^{C/p} \underset{j}{max} \{ w_{i*p + j + s \cdot C} \}) / p$.}


==> texts/tree-schemes.tex <==
\section{Parallel Tree-based Statistical Analysis}
\label{sec:tree-schemes-for-statistical-analysis}

% \subsection{Background on Tree-based Statistical Analysis}
% \label{ss:background-statistical-analysis}

The theoretical efficiency and effectiveness of BHA over lattice models are evidenced by statistical analyses under varied prevalence and individual risk levels. Statistical analysis is conducted by exhaustively constructing all possible test sequences in a tree style up to a certain depth (referred to as the number of \textit{stages}) based on generating test selections using BHA and updating the posterior probability distributions along branches. Classification performance statistics for Bayesian-based group testing methods can be evaluated on this tree, including the rate of decisive classification, as reflected by stringent posterior error threshold(s) being satisfied, false positives/negative rates, and the expected number of tests. 

The process of constructing a tree is described as follows: BHA selects one test at the first stage, which can return two possible results: negative or positive. For the negative branch, after the root lattice model updates its posterior probability distribution based on the negative response, a second-stage BHA can be performed. This holds similarly for the positive branch at the first stage. Therefore, this tree can be spawned like a fully-grown binary tree, and each branch formulates a test sequence. A typical statistical analysis can reach 24 stages comprising up to $2^{24}$ (over 16 million) branches.

% \vspace{-1.0ex}
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/architecture-multi-tree.pdf}
         \caption{The multi-tree scheme proposed by \cite{tatsuoka_bayesian_2022}}
         \label{fig:architecture-multi-tree}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/architecture-single-tree.pdf}
         \caption{The single-tree scheme}
         \label{fig:architecture-single-tree}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/architecture-fusion-tree.pdf}
         \caption{The fusion-tree scheme}
         \label{fig:architecture-fusion-tree}
     \end{subfigure}
        \caption{Parallel Tree Construction Schemes}
        \label{fig:architecture-tree-schemes}
\end{figure*}

% \vspace{-2.0ex}

\subsection{Existing Approach: The Multi-tree Scheme}
\label{ss:multi-tree}
The existing study\cite{tatsuoka_bayesian_2022} proposes a tree construction approach named the multi-tree scheme, which divides the big tree into multiple small trees that each correspond to one true state. The statistical reasoning behind this scheme is that for a given true state, most of the branches in the tree are statistically non-significant and can hence be pruned; we name this technique as \textit{branch pruning}. For example, the branch \{$<$ABC, Positive$>$, $<$A, Positive$>$, $<$C, Positive$>$, $<$B, Positive$>$\} is practically impossible given the true state $ABC$ (subject $A$, $B$, and $C$ are all negative), whereas it is statistically sound if the true state is $\hat 0$ (subjects $A$, $B$, and $C$ are all positive). Therefore, each tree will be drastically smaller.

The benefit of the multi-tree scheme is the easiness of parallel construction. Figure~\ref{fig:architecture-multi-tree} depicts the parallel architecture for the multi-tree scheme with four nodes (one master and three workers). It uses \textit{inter-tree parallelism}, where each worker can independently perform tree constructions. Since each tree can expand differently, this technique also adopts a fine-grained task scheduling protocol to achieve load balance, leading to a claimed scaling efficiency of up to 99.5\% using up to 896 cores.

Despite being easy to parallelize, we find three drawbacks in the multi-tree schemes compared to constructing only one big tree. \textit{First}, the multi-tree scheme has a much higher asymptotic complexity because the number of required trees will grow exponentially as $N$ increases, whereas the size of the single tree is bounded and independent of $N$, e.g., a 24-stage tree contains up to $2^{24}$ branches no matter the $N$. \textit{Second}, the multi-tree scheme is inefficient, as trees can share the same partial branches that resort to duplicated computation. \textit{Third}, the multi-tree scheme does not unleash the full optimization potential of the lattice shrinking technique (see \S\ref{ss:bitwise-operations}). The multi-tree scheme has to start each tree from the initial, full-size lattice model. As a comparison, in the big tree, the initial lattice model is only constructed once and will be quickly shrunk along branches. Therefore, the big tree typically comprises fewer full-size and large-size lattice models.

To alleviate the first drawback, the existing study\cite{tatsuoka_bayesian_2022} proposed two mathematical optimizations to reduce the number of constructed trees: 1) the symmetry property of the lattice model can reduce the number of required trees from $2^N$ to $N+1$ if individual risk levels are homogeneous, namely \textit{the symmetry approach}; and 2) by discarding true states with low prior probabilities up to certain percentage, e.g., 0.1\% total, the multi-tree scheme can retain 99.9\% statistical accuracy while significantly reduce the number of true states that requires evaluation, namely \textit{the accuracy trade-off approach}. Regardless, these two approaches trade off generality or accuracy vs. performance, which we consider not ideal for SBGT. As for the second and the third drawback, the existing study did not provide a viable solution, possibly limited by the multi-tree scheme's innate deficiency.

\subsection{The Single-tree Scheme}
\label{ss:single-tree} 

Based on the multi-tree scheme's drawbacks, we propose constructing the big tree in parallel, namely \textit{the single-tree scheme}. Figure \ref{fig:architecture-single-tree} depicts the single-tree scheme's parallel architecture using four nodes. Unlike the multi-tree scheme, which uses depth-first construction for each tree, the single-tree scheme adopts a breadth-first approach to construct the big tree stage by stage. This allows each worker to perform the test selections (Line 6 to 29 of Algorithm~\ref{alg:test-selection}) for a portion of lattice models at the current stage by \texttt{map()} all lattice models as a resilient distributed dataset (RDD), namely \textit{inter-lattice parallelism}. After test selections are complete, the master use \texttt{collect()} call to gather every updated lattice model and append it to the corresponding location of the tree. The master then schedules tasks for the next-stage tree construction until reaching the maximum stage. 

The issue with exclusively using inter-lattice parallelism for the single-tree scheme is that it leads to insufficient degrees of parallelism during the beginning stages, e.g., even the seventh stage only contains up to 128 lattice models. We propose two solutions to solve this issue: 1) we use intra-lattice parallelism (see \S\ref{ss:parallel-test-selection}) to achieve full resource utilization; and 2) we adopt multithreading on Spark into inter-lattice parallelism, such that each worker node computes Algorithm~\ref{alg:test-selection} instead of Spark's default one CPU core per lattice model. Another issue with inter-lattice parallelism is that when cooperated with lattice shrinking, it can lead to a skewed computation workload because lattice models can vary in size. We hence propose \textit{task alignment}, which organizes the group of lattice models by size and divides it into subgroups; then, each subgroup is sequentially dispatched by the master as a standalone task to ensure load balance. When the number of lattice models in a subgroup does not suffice the degrees of parallelism (usually full-sized or large-sized lattice models), SBGT uses intra-lattice parallelism for this sub-task. 

Our evaluation (see \S\ref{ss:tree-scheme-benchmark}) shows that the single-tree scheme is up to 515x faster than the multi-tree scheme for a medium-scale Bayesian group testing ($N = 17$). Even applying the symmetry approach or the 99.9\% approach, the single-tree scheme still outperforms the multi-tree scheme by up to 1.7x and 54.4x, respectively.

\subsection{The Fusion-tree Scheme}
\label{ss:fusion-tree}

Summarized from the above two tree construction schemes, we raise the question: \textit{Can we leverage each scheme's advantages and alleviate its drawbacks by creating a deep fusion of the two?} The answer is yes. We propose a scheme named \textit{the fusion-tree scheme}. The key idea is that after the single-tree scheme finishes constructing every big tree stage, we perform the identical branch pruning process in the multi-tree scheme. As demonstrated in Figure~\ref{fig:architecture-fusion-tree}, the branch in Worker 3 is pruned, which reduces future computation workload and data communication overhead to the fusion-tree scheme. The statistical reasoning behind branch pruning in constructing a single tree is that some low-probability branches, such as \{$<$A, Positive$>$, $<$A, Negative$>$, $<$A, Positive$>$, $<$A, Negative$>$, $\cdots$\} are statistically meaningless to any true states, hence should be pruned immediately. From the computational perspective, pruning low-statistics lattice models at an early stage prevent lower-statistics lattice models from spawning in later stages, reducing the computation workload in the long run. Also, the lattice shrinking technique usually works poorly along such branches, which leads to computation on unnecessary large-sized or even full-sized lattice models. Last but not least, extending branches is computationally costly, which necessitates the construction of new lattice models and computations of test selections, while branch pruning is computationally efficient and as easy to parallelize as the multi-tree scheme.

Our evaluation (see \S\ref{ss:tree-scheme-benchmark}) shows that the fusion-tree scheme successfully improves statistical analysis speed on large-scale Bayesian group testing ($N = 25$) over the single-tree scheme by up to 7.7x, as it leverages advantages and avoids disadvantages from both the multi-tree scheme and the single-tree scheme. It also offers the best architectural optimization to computational efficiencies and memory footprint in our implementations, which helps SBGT push the efficiency and performance of statistical analyses to the edge.


==> texts/zebraconf+sbgt-backup-text.tex <==
\section{Motivation And Problem Statement}

\textcolor{red}{In the first subsection, you need to state what the problem is, like your motivation, why this problem is important, and why solving it (with our solution) can bring transformative benefits to the field. In the next subsection, you need to formally define this problem as a computer science problem (like using algorithms or figures to illustrate the process/workflow) and highlight what our design will play in the whole process.}

\subsection{Motivation}
In today’s fast-paced software development landscape, the rapid evolution of systems requires frequent detection of heterogeneous unsafe parameters in updated software configurations. As distributed systems increasingly adopt heterogeneous configurations to optimize performance and adapt to changing workloads, the risk of errors increases. Identifying these unsafe parameters is crucial to ensure system stability, prevent communication failures, and maintain consistent behavior across nodes in dynamic, large-scale environments. Currently, ZebraConf provides a solution for identifying such parameters. However, we identified three major limitations of ZebraConf that hinder its ability to perform frequent and reliable testing.

\textbf{First, ZebraConf employs an inefficient group testing strategy.} ZebraConf binary-splitting-based group testing strategy begins by subjecting all parameter configuration tuples in a testing group to an initial unit test. If this test returns positive, the group is split into two subgroups, each undergoing further independent unit tests. This approach lacks efficiency and requires additional processes to reduce false outcomes.

\textbf{Second, ZebraConf lacks an effective method for reducing false outcomes.} For false positive, ZebraConf implements hypothesis testing to reduce false positives. Hypothesis testing occurs when a unit test with one parameter with a heterogeneous configuration returns a positive outcome.  In this process, ZebraConf conducts multiple runs of the unit test, comparing results from both heterogeneous and homogeneous configurations of the candidate. This method increases testing time, requiring repeated unit tests to classify a single parameter.
For false negatives, Zebraconf does not have a systematic way to reduce false negatives.

\textbf{Third, ZebraConf does not consider parameter dependency in testing.} ZebraConf treats heterogeneous parameters as unsafe only when they are tested individually and does not consider the influence of interdependent parameters. This constraint can produce false negatives. Certain parameter configurations might test positive when tested as a group but test negative if tested individually. the binary splitting strategy fragments these combinations, leading ZebraConf to conclude that no heterogeneous unsafe parameters exist within the group

\subsection{Problem Statement}
These insights raise a fundamental research question: Can we develop software that minimizes computational costs while improving the detection accuracy of heterogeneous unsafe parameters? To address this question, we design and implement BsoZebraConf with its core idea illustrated in Figure 1 

We formally define our goal as follows:
\begin{itemize} 
\item \(C \): Denotes the computational cost of classification. 
\item \(A \): Denotes the accuracy of the classification. 
\item \( \theta_i \): represents the i-th set of hyperparameters for the Bayesian test selector. 
\item \( F_i \): Denotes the i-th configuration file. 
\item \( \text{Conf}(F_i) \): Represents the heterogeneous parameter configuration based on the configuration file \( F_i \).
\item \( \lambda \): Weight parameter balancing the trade-off between computational cost and accuracy.
\end{itemize}

\[
\min \sum_{i=1}^n \left( C(\theta_i, \text{Conf}(F_i)) + \lambda A(\theta_i, \text{Conf}(F_i)) \right)
\]

By reducing computational costs, frequent testing becomes feasible. We can improve system stability through configuration changes or updates. Minimizing the false rate reduces waste resources on unnecessary fixes and ensures critical issues are not overlooked.

\section{Design}
This section introduces/discusses XXX.

\textcolor{red}{figure for design}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{szfigures/BsoZebraConf.drawio.pdf}
    \caption{Overview of BsoZebraConf. }
    \label{fig:enter-label}
\end{figure}
% \vspace{-2.0ex}
\subsection{Overview}
The integration of Bayesian approaches with ZebraConf involves three primary modules: 
\subsubsection{Bayesian optimization (BO) module}
Consists of a Bayesian optimization-based hyperparameter selection process before the main testing process and a Bayesian optimization daemon that runs in the background of the main testing process. This module automates hyperparameter selection for future heterogeneous unsafe parameter detection. 

\subsubsection{Bayesian Group Testing (BGT) Module}
Consists of a lattice model that captures the probability distribution of each parameter being erroneous and a Bayesian test selector that the lattice model guides to choose the next parameter combination to test. This module systematically tests the parameters to increase efficiency while reducing the false rate.

\subsubsection{Test Execution module}
Consists of StateTestRunner, which tests the selected parameter in heterogeneous configuration. The test results will update the lattice model. 

\subsection{Design of Bayesian Optimization Module}
Bayesian optimization (BO) navigates the Bayesian test selector's hyperparameter search space to identify the optimal combination tailored for ZebraConf's test set. This optimization process leverages the Gaussian Processes surrogate model and the Expected Improvement acquisition function to efficiently explore the high-dimensional search space, narrowing down to a hyperparameter combination that yields the best performance for the target testing set.

Running the entire test set for every iteration of Bayesian optimization would yield the most accurate results for determining the optimal hyperparameter combination. However, executing the full test set at each iteration would require substantial time and resources, especially given that BO often requires many iterations to thoroughly explore a high-dimensional search space. 

To solve this challenge, we introduce Bayesian optimization Daemon and separate the full test set into two phases: Exploration phase and Exploitation phase with Bayesian Optimization Daemon.



\subsubsection{Exploration phase}
The first 200 unit files in the full test set are for the Exploration Phase, where Bayesian optimization is run continuously. During each iteration of Bayesian optimization, a hyperparameter combination is suggested. This set is tested on the files from the i*10th to i+1*10th positions in the test set to reduce possible bias induced by a small test set. By systematically exploring the search space in the initial stages, we build a surrogate model that accurately reflects the entire test set.

\subsubsection{Exploitation phase with Bayesian Optimization Daemon}
The remaining unit test files, following the first 200, are for the Exploitation Phase. In this phase, the best hyperparameter combination identified during the Exploration Phase is used to test the unit tests. Occasionally, during the Exploitation Phase, the Bayesian Optimization Daemon will propose a new hyperparameter combination based on existing data to test on a subset of 10-unit test files. If the new hyperparameter combination is better than the current hyperparameter, the Bayesian test selector will use the new hyperparameter for future testing. This ensures we continue exploiting the best-known combination while also exploring the space further to identify potentially better hyperparameter combinations.

Through our approach, we automate the hyperparameter selection process for the Bayesian group testing module. 

\subsection{Design Of Bayesian Group Testing Module}
In the middle layer, a lattice model is constructed using prior probabilities of each parameter being erroneous. These prior probabilities reflect expert understanding of parameter behavior and their potential impact during execution. The lattice model will be updated after each unit test execution. The Bayesian test selector analyzes the lattice model and selects a lattice state, representing a parameter combination that can give the most informative result after testing. The selected state is decoded by StateTestRunner for execution.

There are two key designs in the Bayesian Group Testing Module:

\subsubsection{Global Prior Probability Mapping for Parameter Classification}
To capture the classification history and ensure a systematic classification of the potential heterogeneous unsafe parameters, we introduce a global prior probability mapping for each parameter. At the start of the full test run, each parameter is assigned a prior probability based on expert knowledge. Since parameters can appear in multiple unit tests, after each classification, if a parameter is classified as heterogeneously unsafe, its prior probability for subsequent tests is increased. Conversely, if a parameter is classified as negative, its prior probability decreases.

This approach allows us to leverage the observations from previous tests, accelerating future evaluations of the parameter. Moreover, it enables a more sophisticated classification process at the end of the full test run. By analyzing the prior probabilities associated with each parameter at the conclusion of the classification, we avoid making decisions based on a single observation. Instead, we adopt a holistic view of the parameter’s behavior across all classifications.

\subsubsection{Handling Parameter Dependencies and Reducing False Positives}
ZebraConf’s binary splitting strategy fragmented parameter combinations; configuration parameters are flagged as unsafe when tested individually, without accounting for interdependencies between parameters. This can lead to false positives: when parameters are tested in combination, they may return a positive result, but when split into subgroups, each returns negative, which contradicts the initial outcome. For instance, if configuration parameters \{A, B, C\} are tested together and yield a positive result, but testing \{A, B\} and \{C\} separately results in negatives, this inconsistency indicates a potential dependency between parameters.

To address this, we track the state of each test selection. The Bayesian test selector will take account of the inconsistent behavior and reselect the original combination \{A, B, C\} and its subsets for further testing. If inconsistent behavior persists after a predetermined number of iterations, \{A, B, C\} will be flagged as having a dependency relationship and saved for manual interpretation to confirm the nature of their interaction. This approach reduces false negatives that are introduced by fragmenting the parameter dependency, which improves system security. 

\subsection{Design of test execution module}
At the bottom layer, the StateTestRunner interprets the selected lattice state and generates a group testing tuple consisting of only the relevant parameters. This tuple is then used to execute a unit test, where each parameter in the group testing tuple is heterogeneously configured. The test results will update the lattice model. This iterative process continues until the lattice state reaches a predefined probability threshold, as dictated by the hyperparameter.

% \subsection{Enhancements} % remove

\textcolor{red}{For each design, why is this design important, what's the challenge of tackling it, why and how we approach it, what is the challenge of using our approach to address it, what's the outcome of our approach}

% \textcolor{red}{make section title be more informative}
% \subsubsection{Group Test Efficiency}
% The first enhancement addresses ZebraConf’s binary-splitting-based group testing strategy. Currently, ZebraConf begins by subjecting all parameter configuration tuples in a testing group to an initial unit test. If this test returns positive, the group is split into two subgroups, each undergoing further independent unit tests. Each positive subgroup is repeatedly divided and tested until either a subgroup returns a negative result or a positive subgroup is reduced to only containing a single parameter configuration tuple. This approach is efficient if all tuples are negative, requiring only one test. However, when positive tuples are present—especially if they are widely separated—multiple rounds of testing are needed. By integrating Bayesian test selection we aim to optimize the testing process, reducing test repetitions and improving efficiency in scenarios with distantly separated positive tuples.
% \subsubsection{Minimize False Outcome}
% The second enhancement focuses on addressing ZebraConf’s current limitations in minimizing false outcomes. At present, ZebraConf’s binary splitting strategy lacks an effective method for reducing false negatives. Suppose a unit test involving a true positive parameter returns negative at any stage in the tree. In that case, the binary splitting approach will incorrectly conclude that no positives exist within this subgroup, resulting in a false negative outcome. ZebraConf implements hypothesis testing to reduce false positives when a unit test returns positive for a group containing only a single candidate, meaning only one of its parameters is configured heterogeneously. In this process, ZebraConf conducts multiple runs of the unit test, comparing results from both heterogeneous and homogeneous configurations of the parameter in question. By rejecting the null hypothesis that the parameter is heterogeneously negative only if results meet a specified confidence threshold, this approach enhances detection accuracy. However, this method increases testing time, requiring repeated unit tests to classify a single parameter. 
% \subsubsection{Parameter Dependency}
% The third enhancement addresses a key limitation in ZebraConf’s current approach to identifying heterogeneous unsafe parameters. Currently, ZebraConf treats heterogeneous parameters as unsafe only when they are tested individually and does not consider the influence of interdependent parameters. This constraint can produce false positives: certain parameter configurations might test positive when assessed as a group but test negative if tested individually. The binary splitting strategy exacerbates this by fragmenting these combinations, which leads ZebraConf to conclude that no heterogeneous unsafe parameters exist within the group. To overcome this limitation, we introduce a refined analysis strategy that evaluates configurations by considering both individual settings and the interactions between parameters. This enhancement reduces false positives, providing a more accurate detection of heterogeneously unsafe configurations.

\textcolor{red}{emphasis on engineering effort of adding group testing}

\textcolor{red}{talk about modularization}

% \subsection{Bayesian Group Testing’s advantages}
% Baysian group testing has advantages over binary splitting in many aspects.
% \begin{itemize}
% \item Accuracy and Efficiency. One of the key strengths of SBGT is its almost certain convergence to the ground truth, achieving optimal rates of convergence. This holds even in situations characterized by high prevalence rates [2]. Additionally, SBGT distinguishes itself by incorporating the developer's domain-specific prior knowledge into the testing process. This knowledge is translated into prior probabilities, which can facilitate even faster group testing classifications [2]. By integrating this prior information, Bayesian Group Testing can adjust its strategy dynamically, focusing testing efforts where they are most likely to yield informative results to reduce the overall number of tests required
% \item Robustness. SBGT acknowledges testing errors through response probability distributions that can reflect subject correlations at the per-subject level. By incorporating such detailed probabilistic considerations, SBGT significantly reduces the incidence of both false positives and false negatives [2].
% \item Flexible and Comprehensive. SBGT has many parameters that can be adjusted [2]. For example, we provide adjustments in classification thresholds to control false rates. We provide an exhaustive statistical analysis workflow to examine the best settings of tunable parameters in ZebraConf’s context.
% \end{itemize}

\section{Implementation}
\textcolor{red}{Three subsections: one discusses integration-related implementation in ZebraConf so it can seamlessly adopt BGT, basically what we did to make ZebraConf work well with BGT. The second subsection is the implementation of BGT and how prior information is incorporated (I think we have a lot of small tweaks and findings). The third subsection should be Bayesian optimization implementation.}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\SetKwComment{Comment}{$\triangleright$ }{}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\newcommand{\algrule}[1][.8pt]{\par\vskip.25\baselineskip\hrule height #1\par\vskip.25\baselineskip}
\SetKwProg{myproc}{Procedure}{}{}
\SetKwProg{mysubroutine}{Subroutine}{}{}

\begin{algorithm}
\small
\DontPrintSemicolon
  \KwInput{Hyperparameters $H$, Candidates $C$, Unit Test $U$}
  \KwOutput{Classification Result}
  
  \algrule
  \nonl \textit{Main loop} \;
  \algrule
  \myproc{\proc{BGT\_HCONF\_TEST($H$, $C$, $U$)}}{
    $Priors \gets \proc{Get\_Priors\_Based\_On\_Candidates($C$)}$ \;
    $Lattice \gets \proc{Build\_Lattice\_Model($H$, $Priors$)}$ \;
    
    \While{\textbf{not} $Lattice.Classified()$}{
        $Selected\_State \gets Lattice.Select\_State\_To\_Test()$ \;
        \If{$\proc{Detect\_Loop($Lattice.History$)}$}{
            Record The Dependency Loop And Terminate\;
        }
        $Unit\_Test\_Result \gets \proc{State\_Test\_Runner($Selected\_State$, $C$,$U$)}$ \;
        $Lattice.Update\_Posterior\_Probability($Selected\_State, $Unit\_Test\_Result$)$ \;
        $Lattice.Shrink\_If\_Possible() \;
    }
    \Return{$Lattice.Classification()$} \;
  }
% \mysubroutine{\proc{State\_Test\_Runner(selected\_state, $C$, $U$)}}{
%     $group\_test\_tuple \gets []$ \Comment*[r]{\textnormal{Initialize empty group}}
%     \For{$i \gets 0$ to $\text{size of $C$} - 1$}{
%         \If{$(selected\_state \& (1 << i)) > 0$}{
%             Append $candidates[i]$ to $group\_test\_tuple$ \;
%         }
%     }
%     \Return{$HConfRunner.runTest(unit\_test, group\_test\_tuple)$}
% }

  
  \caption{BGT Guided Heterogeneous Configuration Testing}
  \label{alg:bgt-Hconf-test}
\end{algorithm}

\subsection{Integration of ZebraConf with Bayesian group testing}
To integrate heterogeneous configuration testing with Bayesian group testing, we implement the process outlined in Algorithm 1. The process begins by determining prior probabilities based on the testing candidates. These probabilities are then combined with hyperparameters optimized through Bayesian methods to construct the lattice model. Once the lattice is built, the main testing loop begins.

Within the loop, the Bayesian test selector identifies one lattice state, representing a specific parameter combination to test. Before running the unit test, the function checks the test history for any repeated or inconsistent outcomes that could indicate a dependency relationship between parameters. If no such dependency is found, the StateTestRunner decodes the lattice state into parameter groups and executes the unit test, configuring the selected parameters heterogeneously. The loop continues until all parameters in the lattice model are successfully classified.

We introduce the following additional implementations to seamlessly integrate ZebraConf with Bayesian Group Testing (BGT):

\subsubsection{Directory Corruption Backup}
During certain unit test runs, specific parameters configured with invalid values can permanently alter the unit test directory and the ConfAgent settings, resulting in a corrupted testing environment. This corruption has significant downstream effects, as it causes future unit tests—executed on non-heterogeneous, safe configurations with otherwise valid parameter values—to fail erroneously. Such failures compromise the reliability of the testing process and result in solely positive test results.
To address this issue, we implemented a backup and restore mechanism. Before each unit test, a snapshot of the test directory and associated configurations is created, preserving a clean and valid state. Once the unit test completes, the directory is restored to this original state, effectively isolating any effects of invalid configurations and preventing them from impacting subsequent tests. This approach not only safeguards the integrity of the test environment but also enhances the accuracy of results, ensuring that future tests run in a consistent and stable configuration.
By reverting to the backed-up state after each test, we maintain a controlled testing environment where parameters are evaluated independently, without residual interference from prior configurations. This strategy significantly improves testing efficiency and reliability, making it a foundational step in ensuring accurate and meaningful results from the unit test suite.
\subsubsection{Filtering}
In our evaluation of preliminary test results, we identified that a small subset of parameters causes the majority of invalid value failures—those unrelated to configuration heterogeneity. This insight allows us to streamline the testing process by filtering out configuration tuples that include these high-failure parameters, significantly reducing unnecessary test iterations. 
We drastically decrease the testing time without compromising result quality by excluding tuples with these problematic parameters. While this approach requires a few parameters to be flagged for manual interpretation, the trade-off is a considerable boost in testing efficiency and resource utilization. This filtering method not only accelerates the process but also allows the lattice model to focus on configurations that are more likely to reveal meaningful outcomes, ultimately enhancing the robustness and practicality of the testing workflow.
We introduce a post-testing filtering step to address issues with invalid values in testing tuples that lead to unit test failures for heterogeneously safe parameters. After running the Bayesian-Selection test in a heterogeneous configuration, any parameters causing test failures are flagged for further analysis.
In this step, we evaluate the test results for each parameter in the tuple. If a parameter passes the unit test in a homogeneous configuration but fails in the heterogeneous one, it is marked as a false positive due to invalid values. These parameters are excluded from the final result set, ensuring that only heterogeneous unsafe configurations are flagged.

\subsection{Implementation of BGT Module}
\subsubsection{Prior probability}
To further improve the efficiency of the testing process, we incorporate domain knowledge about the parameters by assigning different prior probabilities during the lattice model construction. Based on empirical observations and expert knowledge, certain parameters are intuitively more likely to pose a higher risk of being heterogeneously unsafe. Examples include parameters related to encryption, resource allocation, and network configurations, which were identified as high-risk due to their complexity and variability in different environments.
To reflect this understanding, we create a list to hold high-risk parameters. During the lattice model's initial construction, parameters included in this high-risk list are assigned distinct prior probabilities, distinguishing them from the rest of the parameters. By assigning higher initial probabilities to these parameters, the model focuses more resources on exploring and testing configurations that are more likely to fail, thereby improving the efficiency of the search process and reducing the likelihood of overlooking critical failures.
\subsubsection{In-place Lattice shrinking}
The lattice shrinking enhancement allows Bayesian test selection to optimize testing efficiency by removing candidates from further testing once they’ve been classified. Specifically, when the upset posterior probability mass of a candidate in the lattice model meets the preset classification threshold, that candidate—and all associated states in the lattice model—are removed, effectively reducing the lattice size by half. 
Unlike the original SBGT approach, which reconstructs lattice models for tree-based statistical analysis, we adopt a single lattice model throughout the classification of the entire test pool. This saves time by eliminating the need for repeated lattice reconstruction. To implement in-place lattice shrinking, we directly update the posterior probability map by deleting states that contain the classified candidate. The posterior probabilities of removed states are redistributed to equivalent states, representing the group without the classified candidate, thus preserving the statistical integrity of the model.



\subsection{Implementation of Bayesian Optimization}
SBGT has 6 parameters that can be customized to suit every test set. 
\begin{itemize}
\item \textbf{MaxPoolSize}: maximum number of candidates in a single BGT test pool. Low: 10 High: 20
\item \textbf{DefaultPrior}: prior probability for all candidates. Low: 0.00001, High: 0.2 (lower value indicates that the candidate is initially assumed to have a lower possibility of being positive)
\item \textbf{KnowPrior}: prior probability for candidates that appear in the “high positive probability candidate list” Low: 0.000001, High: 0.99999
\item \textbf{UpTheshold}: the up threshold for BGT classification Low: 0.000001, High: 0.01 (the threshold used for BGT classification. A lower value requires more testing before a state can be classified)
\item \textbf{DownTheshold}: the down threshold for BGT classification Low: 0.000001, High: 0.01 (the threshold used for BGT classification). A lower value requires more testing before a state can be classified)
\item \textbf{Dilution}: enable dilution matrix calculation if above 0.5 Low: 0, High:1 
\end{itemize}
Manually searching through six dimensions of parameters to find the optimal combination for each test set is highly time-consuming. To mitigate this, we automate the process by leveraging Bayesian optimization (BO) to fine-tune the six key parameters of SBGT that best fit each test set, significantly reducing tuning time.

During each iteration of Bayesian optimization, we run 10 Docker containers to evaluate 200 candidate configurations in parallel. Each container runs on different core pairs to prevent resource thrashing and maximize efficiency. Upon completing the tests, the total test time and total test count are compared to ZebraConf's original benchmark of 8050 seconds and 368 tests, respectively. Using this data, we compute two metrics: time-saving normalized and test-count-saving normalized. These metrics form the basis for calculating the objective function, which guides the optimization process.

\begin{figure}[h]
    \centering
    \[
    0.4 \cdot \text{TSN} + 0.4 \cdot \text{CSN} - \text{FPR} - \text{FNR}
    \]
    \caption{Formula for weighted calculation, where TSN is time-saving normalized, CSN is count-saving normalized, FPR is false positive rate, and FNR is false negative rate. Higher coefficients indicate a greater weighting in the calculation.}
\end{figure}

\section{Evaluation}
\label{sec:evaluation}

We assess the performance and accuracy of Bayesian ZebraConf across various iterations of Bayesian optimization with different hyperparameters. Each hyperparameter set is derived from iterations of Bayesian optimization that demonstrated improved performance compared to the previous best, specifically at iterations X = 2, 13, 96, and 179. The results are compared against the original ZebraConf when evaluating 1,000 unit test files, aiming to quantify the performance improvements introduced by the techniques implemented in Bayesian ZebraConf.

\textbf{Experimental setup.} Table~\ref{tab:spec} details the clusters used for evaluating Bayesian ZebraConf.

%\begin{wraptable}{r}{.55\textwidth}
% \vspace{-1.0ex}
\begin{table}[htbp]
\caption{Specification of  Clusters}
\label{tab:spec}
\centering
\footnotesize
\begin{tabular}{lll}
\toprule
\textbf{Cluster}    & Cloudlab   \\ \hline
\textbf{Processor}     & Two Intel Xeon Silver 4114 \\ \hline
\textbf{Clock Speed} & 2.20 GHz   \\ \hline
\textbf{No. of Cores}    &     10   \\ \hline
\textbf{RAM (DDR)}    & 192GB   \\ \hline
\textbf{Storage}      & One Intel DC S3500 480 GB 6G SATA SSD  \\ \hline
% \textbf{OS}           & CentOS Linux release 7.8      & Ubuntu 18.04.1 LTS   \\ \hline
\textbf{Scale}        & 1 node (\textbf{10 cores})  \\ \hline
\end{tabular}
\end{table}
%\end{wraptable}
% \vspace{-1.0ex}


\subsection{Evaluation Time Performance}
\label{ss:lattice-model-benchmark}
This experiment evaluates the Test Time performance of Bayesian ZebraConf across various iterations of Bayesian optimization with different hyperparameters.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.80\linewidth]{szfigures/test_time.png}
    \caption{Comparison of Execution Time Between Bayesian ZebraConf (at Iterations X = 2, 13, 96, 179) and Original ZebraConf for Evaluating 1,000 Unit Test Files. Bayesian ZebraConf achieved execution times of 212,609s, 207,327s, 167,494s, and 153,417s, compared to ZebraConf's 472,503s.}
    \label{fig:test_time}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.80\linewidth]{szfigures/time_save.png}
    \caption{Percentage of Execution Time Saved by Bayesian ZebraConf Compared to Original ZebraConf at Different Iterations of Bayesian Optimization. Savings were 55\%, 56\%, 64\%, and 67\% for iterations X = 2, 13, 96, and 179, respectively.}
    \label{fig:time_save}
\end{figure}

Figure~\ref{fig:test_time} compares the execution time of Bayesian ZebraConf, with different hyperparameters, to the original ZebraConf. Bayesian ZebraConf was evaluated at iterations X = 2, 13, 96, and 179, where it required 212,609, 207,327, 167,494, and 153,417 seconds to evaluate 1,000 unit test files. In comparison, the original ZebraConf took 472,503 seconds. This corresponds to execution time savings of 55\%, 56\%, 64\%, and 67\%, as illustrated in Figure~\ref{fig:time_save}.As we increase the number of iterations in Bayesian optimization, the performance of Bayesian ZebraConf improves consistently, with the rate of improvement gradually diminishing and eventually stabilizing. 
\subsection{Executed Test Count}
This experiment evaluates the Executed Test Count of Bayesian ZebraConf across various iterations of Bayesian optimization with different hyperparameters.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.75\linewidth]{szfigures/test_count.png}
    \caption{Comparison of the Number of Tests Executed by Bayesian ZebraConf (at Iterations X = 2, 13, 96, 179) and Original ZebraConf to Classify 1,000 Files. Bayesian ZebraConf executed 54,850, 54,253, 38,204, and 35,426 tests, compared to ZebraConf's 107,962 tests.}
    \label{fig:test_count}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.75\linewidth]{szfigures/count_save.png}
    \caption{Percentage of Test Count Reduction Achieved by Bayesian ZebraConf Compared to Original ZebraConf Across Iterations X = 2, 13, 96, and 179, with reductions of 49\%, 49\%, 64\%, and 67\%, respectively.}
    \label{fig:count_save}
\end{figure}

Figure~\ref{fig:test_count} compares the number of tests executed by Bayesian ZebraConf, with different hyperparameters, to the original ZebraConf in terms of the number of tests required to achieve classification. Bayesian ZebraConf was evaluated at iterations X = 2, 13, 96, and 179, requiring 54,850, 54,253, 38,204, and 35,426 tests, respectively, to classify 1,000 files. In comparison, the original ZebraConf needed 107,962 tests. This corresponds to test count reductions of 49\%, 49\%, 64\%, and 67\%, as illustrated in Figure~\ref{fig:count_save}. We can see an improvement in efficiency on executed test count similar to execution time. As the number of iterations in Bayesian optimization increases, the Bayesian ZebraConf improves consistently, with the rate of improvement gradually stabilizing. 

\subsection{False Positive And Negative}
This experiment evaluates the false positive and negative rate of Bayesian ZebraConf across various iterations of Bayesian optimization with different hyperparameters.
We define the ground truth as the parameter identified by ZebraConf.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.75\linewidth]{szfigures/false_positive.png}
    \caption{False positive rates of Bayesian ZebraConf's classification evaluated at iterations X=2, 13, 96, and 179, with rates of 14\%, 13\%, 4\%, and 0\%, respectively. The figure highlights the significant improvement in false positive rates as the number of iterations increases.}
    \label{fig:false_positive}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.75\linewidth]{szfigures/false_negative.png}
    \caption{False negative rates of Bayesian ZebraConf's classification evaluated at iterations X=2, 13, 96, and 179, with rates of 4\% at iteration 2 and 0\% for all subsequent iterations. This demonstrates the rapid and sustained reduction of false negatives during the optimization process.}
    \label{fig:false_negative}
\end{figure}
Figures~\ref{fig:false_positive} and~\ref{fig:false_negative} illustrate the false positive and false negative rates of Bayesian ZebraConf's classification under different hyperparameters. Bayesian ZebraConf was evaluated at iterations  X = 2, 13, 96, and 179, with false positive rates of 14\%, 13\%, 4\%, and 0\%, respectively. The false negative rate was 4\% at the first iteration and dropped to 0\% for all subsequent iterations.  These improvements in false positive and false negative rates are directly influenced by the classification threshold of SBGT determined through Bayesian optimization.
A more stringent classification threshold reduces the false classification rate but increases the total execution time and test count required for classification. Conversely, a more lenient threshold decreases execution time and test count but may result in higher false classification rates. By balancing accuracy and efficiency, Bayesian optimization identifies a classification threshold that ensures high accuracy while maintaining computational efficiency.

\section{Conclusion}
Bayesian-ZebraConf demonstrates significant advancements in the field of distributed system configuration analysis by addressing the limitations of existing methods such as ZebraConf. By seamlessly integrating Bayesian Group Testing (BGT) and Bayesian Optimization (BO), the framework introduces a probabilistic, adaptive, and efficient approach to troubleshooting heterogeneous-unsafe configurations. Our results highlight substantial improvements across key metrics. Bayesian-ZebraConf reduces test execution time and test count by up to 67\% while achieving a 0\% false negative rate and significantly lowering the false positive rate to 0\% in advanced iterations. These performance gains showcase the effectiveness of leveraging probabilistic reasoning and dynamic hyperparameter tuning for large-scale system analysis. In the future, we plan to explore other group testing methods to further improve the framework. 


